Detecting Network-based Internet Censorship via Latent Feature Representation Learning

Internet censorship is a phenomenon of societal importance and attracts investigation from multiple disciplines. Several research groups, such as Censored Planet, have deployed large scale Internet measurement platforms to collect network reachability data. However, existing studies generally rely on manually designed rules (i.e., using censorship fingerprints) to detect network-based Internet censorship from the data. While this rule-based approach yields a high true positive detection rate, it suffers from several challenges: it requires human expertise, is laborious, and cannot detect any censorship not captured by the rules. Seeking to overcome these challenges, we design and evaluate a classification model based on latent feature representation learning and an image-based classification model to detect network-based Internet censorship. To infer latent feature representations fromnetwork reachability data, we propose a sequence-to-sequence autoencoder to capture the structure and the order of data elements in the data. To estimate the probability of censorship events from the inferred latent features, we rely on a densely connected multi-layer neural network model. Our image-based classification model encodes a network reachability data record as a gray-scale image and classifies the image as censored or not using a dense convolutional neural network. We compare and evaluate both approaches using data sets from Censored Planet via a hold-out evaluation. Both classification models are capable of detecting network-based Internet censorship as we were able to identify instances of censorship not detected by the known fingerprints. Latent feature representations likely encode more nuances in the data since the latent feature learning approach discovers a greater quantity, and a more diverse set, of new censorship instances.

==> Makefile <==
all: paper.pdf revisionreport.pdf

paper.pdf: \
		paper.tex \
		abstract.tex \
		bg.tex \
		eval.tex \
		intro.tex \
		related.tex \
		summ.tex \
		system.tex \
		threats.tex \
		ack.tex \
		duncan.tex \
		chen.tex 
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper

revisionreport.pdf: \
		revisionreport.tex revisionreport_content.tex
	pdflatex revisionreport
	bibtex revisionreport
	pdflatex revisionreport
	pdflatex revisionreport
	


clean:
	$(RM) *.aux *.log *.spl *.bbl


==> bg.tex <==
\section{Background}\label{sec:background}

\subsection{Data Source: Censored Planet}

A team of researchers from the University of Michigan presented an overview of
\textit{Censored Planet}, which they term an "internet observatory", at the
\textit{ACM SIGSAC Conference on Computer and Communications Security} in
November 2020~\cite{sundara_raman_censored_2020}. Their automated process scans
the Internet from a number of vantage points around the world using a variety
of protocols.  Each scan runs over a two day period, on average, and produces
millions of records. The Censored Planet data is produced by the Quack and
Hyperquack scans, which scan for keyword blocking at the application layer
using the Echo, Discard, HTTP, and HTTPS internet
protocols~\cite{vandersloot_quack_2018,raman_hyperquack-v1_2020}.

The Echo protocol~\cite{postel_rfc_1983} is the primary transport protocol for
Quack. It is well suited as it is simple and predictable.  An Echo server
listens for and establishes TCP connections, and then returns to the sender any
data that it receives. To detect deep packet inspection based censorship, a
message is sent containing a potentially sensitive keyword, such as a fully
qualified domain for a commonly blocked site. Since an Echo server by design
simply returns the data, if the same Echo server is reachable with one payload
and is not reachable with a different payload from the same location, then
network errors can logically be set aside as the cause for the difference in
behavior; censorship is inferred.  If these same requests are repeated from a
different location to the same server in the same time frame and both requests
find the server reachable from that location, a false determination of
censorship in the unreachable location is not likely. If there is either no
response at all, a response that differs from what was sent, or a network error
code, Quack will repeat the probe to a maximum of 5 attempts. The authors of
Quack assert that this is sufficient to differentiate between network issues
and interference.

A natural response to keyword blocking of HTTP traffic is for users and hosts
to switch to HTTPS. However, the typical TLS exchange to begin encrypted
communication includes the unencrypted fully qualified domain of the requested
server in the opening exchange.~\cite{blake-wilson_transport_2006} Hyperquack
detects keyword blocking of HTTPS traffic by requesting the \textit{incorrect}
server name from previously profiled HTTPS servers maintained by organizations.
The profile created for each target establishes how that endpoint
characteristically sends an error response for requesting a domain not served
by that endpoint.  HyperQuack then requests a domain name that is being tested
for censorship and compares the response.  Responses that differ from the
expected, profiled response indicate possible tampering.  HyperQuack is
therefore able to detect censorship that is particularly targeting HTTPS
traffic.

A sample Quack data record is shown in Figure \ref{example-echo}.  If the probe
receives a response that does not match the template for the query, the result
set also includes a \textit{Response} object which contains the HTTP headers,
the HTTP response code, the body of the response, and any TLS information from
the response.


\begin{figure}[hbt]
\begin{minted}[linenos,tabsize=2,breaklines,fontsize=\footnotesize]{js}
{
  "vp": "114.116.151.108",
  "location": {
    "country_name": "China",
    "country_code": "CN"
  },
  "service": "echo",
  "test_url": "666games.net",
  "response": [
    {
      "matches_template": false,
      "response": "HTTP/1.1 403 Forbidden\nContent-Type: text/html; charset=utf-8\nServer: ADM/2.1.1\nConnection: close\nContent-Length: 520\n\n<html>\n\t<head>\n\t\t<meta http-equiv=\"Content-Type\" content=\"textml;charset=GB2312\" />\n\t\t<style>body{background-color:#FFFFFF}</style> \n\t\t<title>\u975e\u6cd5\u963b\u65ad222</title>\n\t\t<script language=\"javascript\" type=\"text/javascript\">\n         window.onload = function () { \n           document.getElementById(\"mainFrame\").src= \"http://114.115.192.246:9080/error.html\";\n            }\n\t\t</script>   \n\t</head>\n\t<body>\n\t\n\t\t<iframe style=\"width:100%; height:100%;\" id=\"mainFrame\" src=\"\" frameborder=\"0\" scrolling=\"no\"/>\n\t</body>\n</html>\n",
      "start_time": "2021-07-19T01:07:35.692415469-04:00",
      "end_time": "2021-07-19T01:07:37.135588863-04:00"
    },
    {
      "matches_template": false,
      "response": "HTTP/1.1 403 Forbidden\nContent-Type: text/html; charset=utf-8\nServer: ADM/2.1.1\nConnection: close\nContent-Length: 530\n\n<html>\n<head>\n<meta http-equiv=\"Content-Type\" content=\"textml;charset=GB2312\" />\n   <style>body{background-color:#FFFFFF}</style> \n<title>\u975e\u6cd5\u963b\u65ad120</title>\n  <script language=\"javascript\" type=\"text/javascript\">\n         window.onload = function () { \n           document.getElementById(\"mainFrame\").src= \"http://114.115.192.246:9080/error.html\";\n            }\n</script>   \n</head>\n  <body>\n    <iframe style=\"width:100%; height:100%;\" id=\"mainFrame\" src=\"\" frameborder=\"0\" scrolling=\"no\"></iframe>\n    </body>\n      </html>",
      "start_time": "2021-07-19T01:07:42.135655432-04:00",
      "end_time": "2021-07-19T01:07:42.591173508-04:00"
    },
    {
      "matches_template": true,
      "start_time": "2021-07-19T01:07:47.59136423-04:00",
      "end_time": "2021-07-19T01:07:49.284425189-04:00"
    }
  ],
  "anomaly": false,
  "controls_failed": false,
  "stateful_block": false,
  "tag": "2021-07-19T01:01:01"
}
\end{minted}
\caption{Example Quack data record}
\label{example-echo}
\end{figure}

\subsection{Semi-automated Data Analysis}\label{subsec:dataanalysis}
The researchers at Censored Planet have been processing their data using
filtering scripts based on features defined by their knowledge of the
censorship domain. Central to their approach has been a set of "block page
fingerprints" which are strings of text found in the HTML of known block
pages.~\cite{ceccio_censoredplanetcensoredplanet_2021}  Responses are processed
via regular expressions to identify matches with these strings.  This
fingerprint matching process has been the primary means of finding censored
responses.  Recently, the Censored Planet team also began rendering the HTML
response into an image, and using an image classifying neural network,
ResNet50, to cluster responses.~\cite{raman_measuring_2020} They then examine a
sample of each cluster to verify block pages, identify new pages and engineer a
new fingerprint. 

The Censored Planet researchers intentionally chose the image of a block page
for processing through ResNet50 because block pages from the same tool can be
    constructed in various languages.  From the researchers' perspective the
    similarity of visual design allows them to ignore the language of the text.
    However, the deep learning models of Natural Language Processing would open
    the features of the text to be sources of insight. In addition, a visual
    inspection of the page even by a deep learning network does not include any
    data from the headers or other metadata surrounding the request and
    response.

\subsection{Numerical Embeddings from Structured Data}

Once a censored response is discovered, a human expert has to determine what
makes that pattern unique.  That determination must then be condensed to a
regular expression as described in Section~\ref{subsec:dataanalysis}. A
response indicating censorship that is substantially similar can easily be
missed if its differences cause it to pass through the screen of regular
expressions.

Other researchers from the University of Michigan, Armin Sarabi and Mingyan
Liu, presented a method of analyzing structured text data at the \textit{ACM
SIGCOMM Internet Measurement Conference} in
2018~\cite{sarabi_characterizing_2018}. Their demonstration cases used network
intelligence data to detect and predict malicious hosts, as well as to find
hidden host attributes. JSON data was transformed into numeric vectors, or
\textit{vectorized}, and then condensed into what they term \textit{lightweight
numerical embeddings} using a Variational Autoencoder neural network.

A Variational Autoencoder uses two deep learning networks to automate the
encoding of features.  Originally designed for image data, one network encodes
the image to a feature vector.  The second network decodes the vector back to
an image.  The Autoencoder learns to effectively encode the features of the
image by comparing the original with the image produced by the decoder.  Sarabi
and Liu used the \textit{lightweight numerical embeddings} produced by their
Variational Autoencoder as the data source for deep learning analysis on the
original data.

Since the Censored Planet data is structured as JSON, this approach could be
used to gain new insights into censorship or uncover instances of censorship
not previously found in this data. The Censored Planet data also frequently
contains natural language. This approach could be further enhanced using
methods from natural language processing.

\subsubsection{Natural Language Processing Methods for Vectorization and Auto-encoding}

The Censored Planet data contains HTTP responses composed of both typical HTTP
headers and HTML markup of text in multiple languages. This multilingual markup
needs to be vectorized so that our machine learning networks can analyze it. A
team of researchers from Facebook AI Research (FAIR) presented a transformer
based, cross-lingual model to the \textit{Association for Computational
Linguistics} in 2020~\cite{conneau_unsupervised_2020}. They named their model
XLM-R for XLM-RoBERTa as it is a descendent of the
mBERT~\cite{devlin_bert_2019} and XLM~\cite{conneau_cross-lingual_2019} models
developed previously.

A transformer model is built exclusively around the idea of an attention score
which is a weight, or importance value for every item in set B, given a member
of set A~\cite{galassi_attention_2021}.  The attention score is intended to
quantify relevance.  When considering a particular word in the first set, what
are the most relevant words in the second? Figure \ref{fig:atten} shows a
visualization of attention scores for a translation system.  In the figure,
higher scores are represented by lighter squares~\cite{bahdanau_neural_2016}.

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.8\columnwidth]{../Shawn Duncan M.A. Thesis/attention_example.png}
    % \Description{A rectangular matrix comparing "This will change my future with my family, the man said" to "Cela va changer mon avenir avec ma famille, a dit l'homme" in which the intersection of pairs such as famille & family are white but famille and man are black.}
    \caption{A Visualization of Attention Scores~\cite{bahdanau_neural_2016}}
    \label{fig:atten}
\end{figure}

Transformers use both "self-attention" in which both sets for calculating
attention are the same, such as the input string on itself, as well as
attention between the input and the proposed output. These attention scores are
processed through a standard linear layer to predict the next item of the
output.

The XLM-R model was trained by the team at FAIR using two terabytes of data in
one hundred languages.  The data was taken from Common Crawl which is a
publicly available dataset of text taken from web pages around the
world.~\cite{common_crawl_what_2022} The XLM-R model vectorizes text by
matching a word from any of the languages it recognizes with a numeric token in
its library.

A Sequence-to-Sequence model (Seq2Seq)~\cite{sutskever_sequence_2014} is
composed of an encoder and a decoder. The encoder is presented with each item
in an input sequence, in order, and produces an encoded vector. The decoder
takes the encoded vector as input and produces an output sequence. The primary
use case for a Seq2Seq model is translation.  Imagine that two persons, A and
B, need to communicate but they do not share a language.  Suppose they find two
other persons, encoder and decoder who are both bilingual with exactly one
unknown language in common. Encoder shares a second language with A and decoder
with B.  So person A speaks to encoder, who translates to the unknown shared
language.  Decoder receives the shared translation and translates it again to
deliver it to person B. When a Seq2Seq model is used to build such a
translator, it is trained using supervised learning with pairs of corresponding
phrases.  The Seq2Seq architecture can be used to create an autoencoder if
instead the output sequence is compared back to the input sequence in the
training process.

\subsection{Sequential Data as Images}

Jeyaprakash Hemalatha and an international team of collaborators brought the
tools of computer vision to the task of analyzing sequential data by completely
synthesizing images from the data~\cite{hemalatha_efficient_2021}.  Their
research objective was malware detection.  Grayscale images can be encoded
using a 1 byte pallet, in which the range from black to white is encoded as an
integer between 0 and 255. Figure \ref{fig:parrot} is an example of such an
image. Hemalatha et al. used the bytes of the binary data file to construct a
grayscale image as if the bytes were pixels (Figure \ref{fig:malware}). They
then approached detection as a classification problem and trained a Densenet
based network to classify multiple malware types.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.45\columnwidth]{../Shawn Duncan M.A. Thesis/Grayscale_8bits_palette_sample_image.png}
    %\Description{A grayscale image of a parrot.}
    \caption{Example grayscale image (1 byte pallet)}
    \label{fig:parrot}
\end{figure}
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.45\columnwidth]{../Shawn Duncan M.A. Thesis/malware.png}
    %\Description{An image that appears to be a randomly distributed collection of pixels of black, white and varying levels of gray.}
    \caption{Malware image constructed from bytes}
    \label{fig:malware}
\end{figure}

The DenseNet architecture is based on the convolutional network architecture
with each convolutional layer receiving not just the prior layer as inputs, but
all prior layers as inputs.~\cite{huang_densely_2017} Although a simple change,
connecting all prior layers prevents gradients from vanishing.  The DenseNet
design is able to match the performance of a much larger standard convolutional
network.  This reduction in model size decreases the computation load resulting
in reduced training time. This design was created for the ImageNet
classification challenge in which each item is sorted into one of 1,000
categories based on the content of the image.~\cite{li_fei-fei_imagenet_2012} 

\section{Research Methodology}\label{sec:research}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/ma_research.eps}
    \caption{Research Overview}
    \label{fig:process}
\end{figure}
In this thesis we extend the methods of processing structured text with neural networks developed by Sarbani and Liu. First we apply our extended approach to the data provided by the Censored Planet researchers, and then apply supervised learning to select censored responses from the data.  In addition, we compare this approach to fine-tuning a DenseNet to select censored responses from the data encoded as grayscale images.

\subsection{Structured Text to Vectors}\label{subsec:text2vec}
The data coming from Censored Planet is stored as tar archives in Google Cloud
storage. This data needs to be transformed into numeric form before it can be
processed by a machine learning network (see Figure \ref{fig:pre-process}). Our
CensoredPlanetFlatten~\cite{shawn_p_duncan_censored_2022} uses the
Webdataset~\cite{aizman_high_2019} developed by NVIDIA to iterate through the
data streaming directly from the cloud storage. Each item was transformed as it
was received in the stream and stored to local files.  We filtered the stream
to include only items marked as anomalies by the Quack probe, which are
responses that do not match the expected Echo protocol response.

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/censored_planet_flatten.eps}
    \caption{Vectorizing JSON data}
    \label{fig:pre-process}
\end{figure}

Each result in the source data is structured as nested JSON, the top level is
the metadata common to all the responses for that particular probe, with all
the unique responses nested in the response key (see Figure
\ref{example-echo}). We flattened each record by iteratively pairing the top
level metadata with each set of response data to create a set that pertains to
a single response. Figure \ref{example-flattened} shows an example of two items
flattened from the record shown in Figure \ref{example-echo}.

\begin{figure}
\begin{minted}[linenos,tabsize=2,breaklines,fontsize=\footnotesize]{js}
[{
  "vp": "114.116.151.108",
  "location": {
    "country_name": "China",
    "country_code": "CN"
  },
  "service": "echo",
  "test_url": "666games.net",
  "anomaly": false,
  "controls_failed": false,
  "stateful_block": false,
  "tag": "2021-07-19T01:01:01",
  "matches_template": false,
  "response": "HTTP/1.1 403 Forbidden\nContent-Type: text/html; charset=utf-8\nServer: ADM/2.1.1\nConnection: close\nContent-Length: 520\n\n<html>\n\t<head>\n\t\t<meta http-equiv=\"Content-Type\" content=\"textml;charset=GB2312\" />\n\t\t<style>body{background-color:#FFFFFF}</style> \n\t\t<title>\u975e\u6cd5\u963b\u65ad222</title>\n\t\t<script language=\"javascript\" type=\"text/javascript\">\n         window.onload = function () { \n           document.getElementById(\"mainFrame\").src= \"http://114.115.192.246:9080/error.html\";\n            }\n\t\t</script>   \n\t</head>\n\t<body>\n\t\n\t\t<iframe style=\"width:100%; height:100%;\" id=\"mainFrame\" src=\"\" frameborder=\"0\" scrolling=\"no\"/>\n\t</body>\n</html>\n",
  "start_time": "2021-07-19T01:07:35.692415469-04:00",
  "end_time": "2021-07-19T01:07:37.135588863-04:00"
},
{
  "vp": "114.116.151.108",
  "location": {
    "country_name": "China",
    "country_code": "CN"
  },
  "service": "echo",
  "test_url": "666games.net",
  "anomaly": false,
  "controls_failed": false,
  "stateful_block": false,
  "tag": "2021-07-19T01:01:01",
  "matches_template": false,
  "response": "HTTP/1.1 403 Forbidden\nContent-Type: text/html; charset=utf-8\nServer: ADM/2.1.1\nConnection: close\nContent-Length: 530\n\n<html>\n<head>\n<meta http-equiv=\"Content-Type\" content=\"textml;charset=GB2312\" />\n   <style>body{background-color:#FFFFFF}</style> \n<title>\u975e\u6cd5\u963b\u65ad120</title>\n  <script language=\"javascript\" type=\"text/javascript\">\n         window.onload = function () { \n           document.getElementById(\"mainFrame\").src= \"http://114.115.192.246:9080/error.html\";\n            }\n</script>   \n</head>\n  <body>\n    <iframe style=\"width:100%; height:100%;\" id=\"mainFrame\" src=\"\" frameborder=\"0\" scrolling=\"no\"></iframe>\n    </body>\n      </html>",
  "start_time": "2021-07-19T01:07:42.135655432-04:00",
  "end_time": "2021-07-19T01:07:42.591173508-04:00"
}]
\end{minted}
\caption{Example rows flattened from the data in Figure \ref{example-echo}}
\label{example-flattened}
\end{figure}

Most of the data fields transformed to numbers in a straightforward manner. Datetime fields in ISO format were transformed to UNIX timestamps. Boolean fields transformed to a 1 or 0. We split the IPv4 address into four sequential integers.

There are two text fields needing a more specialized approach: \textit{test\_url} and \textit{response}. This text needs to be transformed to numbers in a consistent and predictable manner. The \textit{response} field is a particular challenge since it can contain the markup of a block page with text in a variety of languages. We used the XLM-R multilingual transformer~\cite{conneau_unsupervised_2020} model to process this text into numeric tokens. Sarbani and Liu term such a transformation \textit{vectorizing}.

Although XLM-R is fast and skilled at vectorizing multilingual text, it requires a token library with just over 250,000 members.  To reduce the scale of training for our autoencoder, we created our own index of the XLM-R tokens being used as we vectorized the data. This reduced the scale of the token vocabulary for our data down to 6,813 active tokens.

\subsection{Training Data}\label{subsec:training}
We used the Censored Planet collection of regular expressions described in Section \ref{subsec:dataanalysis} to determine if an anomalous response was censorship or a false positive~\cite{sarah_laplante_blockpage_2021}. The result was a large dataset of 1,711,339 anomalous responses containing 215,016 censored, 653,481 uncensored, and 842,842 undetermined items. The labeled data is unbalanced since there are 3 times as many responses identified as uncensored as those censored. We applied an approach of under-sampling the majority class to balance the training dataset whenever labeled data was needed.

\subsection{Encoding Features}\label{subsec:encoding}
The majority of the information that comprises a single row in this dataset is natural language in which the sequential relationships are also data. The IP addresses are sequential as well. Once the rows were vectorized into tensors, we trained a Sequence-to-Sequence Autoencoder model to capture the information contained in these relationships~\cite{raff_inside_2021}. The Seq2Seq model is composed of four machine learning blocks: 
\begin{itemize}
    \item Embedding
    \item Encoder
    \item Decoder
    \item Predictor
\end{itemize}

\subsubsection{Embedding}
\begin{table}[h]
  \caption{Embedding Parameters}
  \label{tab:ae_embed}
  \begin{tabular}{p{0.66\columnwidth} r}
    \toprule
    Parameter & \\
    \midrule
    number of embeddings & $7,069$ \\
    embedding dimension & $96$ \\
    \midrule
    trainable parameters &  $6.78 \times 10^{5}$ \\
    \bottomrule
  \end{tabular}
\end{table}
The Embedding block takes token values and creates a tensor to be processed.  It uses 7,069 possible values for input tokens, which is the largest possible value of the static data, 256, added to the 6,813 token values used from XLM-R. We chose an embedding size of 96 to provide sufficient breadth for computation in the processing blocks after experimenting with the impact on memory requirements and processing time using values between 64 and 128.

\subsubsection{Encoder}
\begin{table}[h]
  \caption{Encoder Parameters}
  \label{tab:ae_encoder}
  \begin{tabular}{p{0.66\columnwidth} r}
    \toprule
    Parameter & \\
    \midrule
    input size & $96$ \\
    hidden size & $128$ \\
    \midrule
    trainable parameters &  $1.73 \times 10^{5}$ \\
    \bottomrule
  \end{tabular}
\end{table}
The encoder in our Seq2Seq implementation is a bidirectional Gated Recurrent Unit (GRU) which processes embeddings as a batch, saving each result as a sequence of states. These states are commonly called \textit{hidden states}.  The final hidden state summarizes the entire sequence. When the Seq2Seq model is properly trained, it is this final hidden state from the encoder that will correspond to Sarbani and Liu's \textit{lightweight numerical embeddings}. As a bidirectional GRU, the functional size of the hidden network is doubled.  We selected 128 for the hidden size. This value multiplies through the decoder and the predictor, exploding memory requirements at higher values. 

\subsubsection{Decoder}
\begin{table}[h]
  \caption{Decoder Parameters}
  \label{tab:ae_decoder}
  \begin{tabular}{p{0.66\columnwidth} r}
    \toprule
    Parameter & \\
    \midrule
    input size & $96$ \\
    hidden size & $128$ \\
    cell layers & $1$ \\ 
    \midrule
    trainable parameters &  $2.71 \times 10^{5}$ \\
    \bottomrule
  \end{tabular}
\end{table}
The complexity of the Seq2Seq model is in the decoder. Before processing an input sequence, we use a simplification of scheduled sampling proposed by Raff~\cite{raff_inside_2021} to randomly choose between \textit{auto-regression} and \textit{teacher forcing} to select the inputs for the decoder. The difference between these strategies begins with the second item of the input sequence. If auto-regression has been chosen the inputs will be sampled from the range of the vocabulary using the probabilities produced by the predictor block.  If teacher forcing is chosen, the decoder inputs are the same as the inputs to the encoder. 

The foundation of the decoder is one or more bidirectional Gated Recurrent Unit Cells, which essentially decomposes the standard Gated Recurrent Unit. This decomposition allows us to calculate attention scores after each token in the input sequence is processed through the GRU cells. Attention scores are computed using a dot product
\begin{equation} \label{eq:1}
score(h_t, c) = \frac{h^T_t \cdot c}{\sqrt{H}}
\end{equation}
with values of $h$ taken from the state produced at step $t$ by the encoder, $c$ is the context, or decoder output at step $t$, and $H$ is the input size used for the GRU Cell. We use the attention scores to calculate a weighted context at each step of the decoding process.

\subsubsection{Predictor}
\begin{table}[h]
  \caption{Predictor Parameters}
  \label{tab:ae_predictor}
  \begin{tabular}{p{0.66\columnwidth} r}
    \toprule
    Parameter & \\
    \midrule
    input size & $512$ \\
    hidden size & $256$ \\
    output size & $7,069$ \\ 
    \midrule
    trainable parameters &  $2 \times 10^{6}$ \\
    \bottomrule
  \end{tabular}
\end{table}
The weighted context is concatenated with the output of the decoder block, and the result is processed by the Predictor block to produce a series of probabilities across the range of possible tokens. These probabilities are then used to compute a cross-entropy loss for each step in the decoding process. The summation of these losses for all decoding steps is used as the loss for the current input. 

\subsubsection{Training}
We trained this model using a randomly selected dataset of 1,197,937 items with an additional 171,134 randomly selected items reserved in a validation dataset. The training was conducted on CPU using a batch size of 2 across a cluster of 8 computing nodes, producing an effective batch size of 16. A large amount of data is an asset for a machine learning network but it is also a challenge if the network is computationally expensive to train. We balanced this asset and constraint by randomly selecting 119,794 items from the training set for use on each epoch. The learning rate varied smoothly between 0.003 and 0.0001.  The network was checked against the validation data following each epoch and the results are shown in Figure \ref{fig:ae_val_loss}. 

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/autoencoder_val_loss.eps}
    \caption{Sequence-to-Sequence Autoencoder Validation Loss}
    \label{fig:ae_val_loss}
\end{figure}

When a Seq2Seq model is trained for translation, standard practice is to evaluate the quality of the training using a Bilingual Understudy score (BLEU) on both a set of validation pairs and a set of test pairs~\cite{papineni_bleu_2001}. Our Seq2Seq model is not used for translation, therefore we set our training objective as a substantial reduction of accumulated loss. We ultimately evaluate the effectiveness of our Seq2Seq model by its ability to produce \textit{lightweight numerical embeddings} that sufficiently summarize the original data for effective training of the classifier discussed in section \ref{subsec:super}. After our network had seen approximately 3,700,160 items in training, the validation loss had dropped below 0.2 of the initial value, which met our training objective.

We continued by using the trained autoencoder to produce two new datasets from our flattened dataset. We first processed the labeled data through the model, under-sampling the uncensored items, to produce a balanced set of labeled \textit{lightweight numerical embeddings} with 215,016 censored items and 214,846 uncensored items.  We then randomly partitioned this data reserving 0.1 of the data for valdiation, 0.2 for testing and the remaining 0.7 for training. We also processed the undetermined items from our flattened dataset as a set of \textit{lightweight numerical embeddings} for later use as an evaluation dataset.

\subsection{Supervised Learning on Lightweight Embeddings}\label{subsec:super}
\begin{table}[h]
  \caption{Lightweight Embedding Classifier Parameters}
  \label{tab:le_params}
  \begin{tabular}{p{0.66\columnwidth} r}
    \toprule
    Parameter & \\
    \midrule
    initial input & 256 \\
    hidden input & 64 \\
    final input & 32 \\ 
    \midrule
    trainable parameters &  $1.86 \times 10^{4}$ \\
    \bottomrule
  \end{tabular}
\end{table}
The fundamental question for any anomaly identified by the Quack probe is, ``Is this anomaly the result of censorship?'' We construct a binary classifier with three layers: an input layer matching the dimension of the embeddings produced by the autoencoder, a hidden layer which condenses the input, and an output layer that further refines the output of the hidden layer to a probability. We then train this classifier using the balanced labeled dataset of \textit{lightweight numerical embeddings}. The learning rate varied between $1 \times 10^{-6}$ and $1 \times 10^{-7}$ using a cosine annealing strategy with period of 10 epochs.  The results are shown in Figure \ref{fig:le_val_loss} and Figure \ref{fig:le_val_acc}. We use early stopping to prevent the classifier from overtraining as the validation loss drops smoothly through the epochs. The trained network resulted in a loss of $0.047$ on the test data with an accuracy of $0.988$.

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/le_val_loss.eps}
    \caption{Lightweight Embedding Classifier Validation Loss}
    \label{fig:le_val_loss}
\end{figure}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/le_acc.eps}
    \caption{Lightweight Embedding Classifier Validation Accuracy}
    \label{fig:le_val_acc}
\end{figure}

\subsection{Densenet}\label{subsec:dense}
Our original flattened dataset was stored as one dimensional arrays.  We determined that the raw bytes of the largest item would fill a square of size (172, 172).  The Densenet algorithm is well known and available as a pre-trained model that expects images sized (224, 224). We reprocessed the flattened dataset by converting each item to bytes, padding each end of the byte sequence with zeros to produce a $224^2$ length sequence and reshaping the result to (224, 224). We produced two datasets in this manner similar to those produced for the Lightweight Embedding Classifier: a balanced labeled dataset with 215,016 censored items and 215,373 uncensored items, as well as a dataset reprocessed from the 842,842 undetermined items.

The Densenet architecture uses a final linear layer as a classifier for the 1,000 image categories.  We replace that linear layer in the pre-trained model with a new layer accepting the same input dimension but producing a single output.  We then resumed training, fine tuning, the model as a binary classifier. The learning rate varied between $1 \times 10^{-6}$ and $1 \times 10^{-7}$ using a cosine annealing strategy with period of 10 epochs. The results of this training are shown in Figure \ref{fig:dn_val_loss} and Figure \ref{fig:dn_val_acc}. The trained network resulted in a loss of 0.048 on the test data with an accuracy of 0.986.
\begin{figure}[hbt]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/densenet_val_loss.eps}
    \caption{Densenet Validation Loss}
    \label{fig:dn_val_loss}
\end{figure}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=\columnwidth]{../Shawn Duncan M.A. Thesis/densenet_val_acc.eps}
    \caption{Densenet Validation Accuracy}
    \label{fig:dn_val_acc}
\end{figure}



==> chen.tex <==
\noindent \textbf{Hui Chen} is an Assistant Professor at the Department of
Computer and Information Science, CUNY Brooklyn College.  He engaged in
geophysical research and worked as a software developer in industry.  His
research experience include projects in mobility management in wireless
networks, caching for wireless systems, coverage problem of wireless sensor
networks, security and privacy, accountable systems and networks, and recommendation systems for
software developers.  He received a Ph.D. in computer science from the
University of Memphis in Memphis, Tennessee.  He is a member of ACM and a
senior member of IEEE. 

==> duncan.tex <==
\noindent \textbf{Shawn P. Duncan} leads a team of software engineers at Memorial Sloan Kettering Cancer Center in New York, NY. He received his B.A. in Mathematics from the University of California, Santa Cruz and his M.A. in Computer Science from Brooklyn College, City University of New York.


==> revisionreport_content.tex <==
\noindent 
We thank the editor-in-chief and the associate editor for handling our paper in
a timely fashion. We owe a great deal of gratitude to the two anonymous
reviewers for their reviews of our paper. 
    
The reviewers pointed out strengths including novelty and contribution of our
paper.  We appreciate these encouraging comments.  The reviewers also indicated
several shortcomings in the paper.  In the following, we summarize our
revisions and our responses to the comments on the shortcomings.  For
convenience, we divided and numbered these comments of the two anonymous
reviewer, e.g., R1.1 is the 1st comment of reviewer \#1 while R2.1 that of
reviewer \#2.  We believe that we addressed and responded all comments on the
shortcomings from the two reviewers.  By addressing these comments we also
believe that we improved the quality of the paper. 




\reviewerno{r1}
\section{Responses to Reviewer \ref{r1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           Comment and Reponse                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\commentno{r1bm}
\subsection{\refcomm{r1}{r1bm}. On Baseline Model}

\comment{%
How realistic is the baseline model used for comparison? Is it being used in
	the industry or proposed by prior work?%
}
\response{
	This is a great question. To the best of our knowledge, our work is the first work 
	that presents an end-to-end automatic Internet censorship detection model. As such,
	a baseline model is not readily available. 

	In order to construct a baseline model, we examined the literature.
	We realized that researchers generally rely on rule-based
	detection methods, sometimes assisted with machine learning algorithms, most of those
	are unsupervised. One example is Niaki et al. who compute page length and 
	term-frequency as data features for each 
	Internet outage response page, cluster the response pages into clusters, and manually examine
	the clusters~\cite{niaki2020iclab}. Another is Raman et al. who encode each Internet response
	page as an image, and use image clustering algorithms to automatically cluster the pages~\cite{raman_measuring_2020}. 

    The motivation for Raman et al.~\cite{raman_measuring_2020}'s image-based data feature 
    representation came from several studies that found the page-length and term-frequency 
    features lead to high false positives for censorship detection~\cite{yadav2018light, 
    raman_measuring_2020}. Raman et al.'s work shows that the image-based feature
    representation yields an improved censorship detection performance in their approach
    combining clustering and manual inspection.
    

	Following the prior works, we design and propose an image-based detection model as
	the baseline model. The feature representation part is identical to that in Raman et al.~\cite{raman_measuring_2020}.
	Upon extracting the features, we use a simple classifier (a multi-layer neural network) to classify the
	response pages. For our autoencode-based end-to-end model, we design an autoencode network to extract
	features, while keeping the classifier identical to the baseline model.

	Considering the above, we believe our baseline model is well justified. To reflect on this justification,
	we revised ``Section 3.4 Alternative Approach'' as follows:
}

\begin{revisiontext}

	Prior works typically adopt a semi-automated approach for Internet censorship 
	detection, where they first leverage an unsupervised machine learning algorithm,
	such as, a clustering algorithm to divide Internet outage measurements, e.g.,
	block pages into clusters, and second, manually examine the clusters to determine
	whether the cluster represents a type of Internet 
	censorship~\cite{raman_measuring_2020, niaki2020iclab}. A necessary step
	in the process is to extract data features from the internet
	measurement data. Page length and term frequency vectors are two features
	borrowed from natural language processing to cluster block 
	pages~\cite{jones2014automated}. Although the clustering algorithm
	using the two features reduces manual efforts to examine the clusters,
	several follow-up studies indicate that the features can lead to 
	high false positives due to natural variations in page length from dynamic
	and language-specific content~\cite{yadav2018light, raman2020measuring}. 
	Recognizing the limitation of the two features, researchers are seeking 
	different feature representation methods for Internet measurement data, such as,
	block pages~\cite{raman2020measuring}.
	
\end{revisiontext}
\vskip 0.5em
\begin{revisiontext}
			
	
	Deep learning has found tremendous success in computer
	vision~\cite{huang_densely_2017, li_fei-fei_imagenet_2012}. In contrast to 
	more traditional learning algorithms, such as, Super-Vector Machine and 
	Tree-based algorithms (Decision Tree, Random Forest) for which we need to
	extract from the raw data manually designed features to represent the data
	in a tabular form, deep learning can learn to extract features directly
	from the raw data, which, numerous studies show it is an advantage because
	we do not always know what the best features might be for a particular 
	machine learning application~\cite{bengio2013representation}. 
	A clever way to
	design a learning system for non-tabular data is to take
	advantage of these recent advances in deep learning by encoding the data as
	gray-scale images and use a deep learning model for computer vision that is
	readily available to learn
	from these images. There have been applications of this approach in several
	domains, such as, for malware detection~\cite{hemalatha_efficient_2021} and for
	software defect prediction~\cite{chen2020software}.  A gray-scale image can be
	encoded using a byte pallet, in which the range from black to white is encoded
	as an integer between 0 and 255. In another words, we can consider a gray-scale
	image as a vector of $W \times H$ integers where $W$ is the width of the image
	and $H$ the height. For our structured data, after converting a
	censorship test record similar to that in Listing~1 into a
	raw vector, we pad the
	beginning and end of the vector with sufficient 0 to 
	equal a uniform length of size $W \times H$. We then export this vector to a
	sequence of bytes, reshape the vector to a $W \times H$ array from which we
	form the gray-scale image.
	
\end{revisiontext}
\vskip 0.5em
\begin{revisiontext}


	Recently several works
	have adopted this approach in their semi-automated censorship detection
	pipeline and find that the approach leads to improved predictive performance
	than those using the page length and term frequency vector 
	features~\cite{raman2020measuring, sundara_raman_censored_2020}. 
	Following these prior works, we build a fully-automated Internet censorship detection model
	where we use images as feature representations of block pages. For this,
	we elect to use the well-known DenseNet
	model~\cite{huang_densely_2017}.  DenseNet uses the architecture of a Convolutional
	Neural Network (CNN). A DenseNet has multiple CNN blocks that have the
	following neuron connectivity pattern: each layer in the CNN block
	is connected to all the others with the block. Due to this connectivity
	pattern, there is a shortcut path between each individual layer to the loss
	function and the training of the layer can be directly supervised by the loss
	function. Aside from this, the connectivity pattern also results in a compact
	network that is less prone to overfitting and encourages heavy feature reuse.
	Because of this, prior work suggests that DenseNet should be a natural fit for per-pixel
	prediction problems~\cite{zhu2017densenet}.
	
\end{revisiontext}
\vskip 0.5em
\begin{revisiontext}

	
	DenseNet is available as a pre-trained model~\cite{pytorchdensenet} 
	that expects images sized $224 \times 224$. The pre-trained model has a final linear
	layer of size 1,000 as a classifier for 1,000 image categories.  We replace
	that linear layer in the pre-trained model with a new layer accepting the same
	input dimension but producing a single output, the probability at which 
	the input is a censorship event.  
	
\end{revisiontext}
\vskip 0.5em
\begin{revisiontext}


	As an alternative to for the proposed End-to-End
	Censorship Detection model (E2ECD), we consider a modeling pipeline as
	illustrated in Figure~2b. For convenience, we refer to
	this model as DenseNetCD. Because the alternative model leverages the feature presentation method
	that prior works consider the best and is equipped with an identical classifier as the
	E2ECD model, we shall use it as a baseline model to compare
	with the E2ECD model. 
\end{revisiontext}

\commentno{r1fi}
\subsection{\refcomm{r1}{r1fi}. On False Identification (Positives and False Negatives)}

\comment{%
Do you explore the data records that are incorrectly identified as censored
	events by the proposed model? And/Or the censored records that are identified
	as normal?%
}
\response{
	This is an excellent question. Perhaps, most relevant is the discussion in 
	``Section 4.5. Censorship Detection on Undetermined Records''. For this, we did
	take a sampling approach, and randomly select several instances in each category
	to gauge its correctness. In the paper, we argue based on our examinations of
	the random samples:

	``Most of the remaining records are likely the result of censorship.  
	An investigation on the
	Great Firewall of China indicates that both \textit{connection reset by peer}
	and \textit{connection timed out} are among its observable
	characteristics~\cite{shu_data_2014}.  As discussed in the above, 
	the response to the request sent to
	these vantage points have been verified with innocuous payloads, and therefore
	it is very unlikely that the network has unexpectedly and repeatedly failed
	during these specific queries.''

	To have concrete understanding about the correctness or the incorrectness of the 
	prediction results, we need to infer both the detection mechanism and the censorship
	intention, which is a task of significant undertaking. Because of this, to make this
	clearer, we added the following paragraph to ``Section 5 Limitations and Threats to Validated''
	under ``Censorship Detection on Undetermined Test Records'':



}

\begin{revisiontext}
	Because the evaluation data set contains in total 842,842 records, a thorough
	examination of the prediction results manually is infeasible. We plan to study
	these test records in a future work. Because we are unable to access people's intention
	who might initiate the censorship events, the correctness of censorship 
	detection is often via cross-examination and inference. For this, we plan to
	compare records collected by multiple Internet censorship measurement 
	platforms including both the Censored Planet and 
	ICLab in the same time period~\cite{sundara_raman_censored_2020,niaki2020iclab}. 
	Second, following the approach adopted by prior works, we shall cluster
	the test records, such as, those predicted as probable censorship events, 
	and manually examine each cluster to determine whether the prediction is correct
	by inferring what the censorship mechanism is and what intention 
	of censorship may be~\cite{jones2014automated,sundara_raman_censored_2020,niaki2020iclab}. 
\end{revisiontext}


\reviewerno{r2}
\section{Responses to Reviewer \ref{r2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           Comment and Reponse                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\commentno{r2mv}
\subsection{\refcomm{r2}{r2mv}. On Motivation}

\comment{%
	To strengthen the motivation of the paper, it would be appropriate to address
	the doubts and preconceptions that a reader who is not familiar with
	censorship might have. For instance, most people would assume that a
	democratic country would rarely apply censorship and if it does, with a
	warrant, it would inform about that. If that were true, why would not simply
	rely on a country or set of `free' countries as the basis for detection?%
}
\response{
	That is an insightful observation. Following this advice, we revised/added several sentences to the Introduction section.
	The relevant text now reads as follows:
}

\begin{revisiontext}
	The network-based Internet censorship can lead to network
outages~\cite{dainotti2011analysis}.  Differentiating the censorship events
from other types of outages can thus benefit the design and implantation of
Internet network architecture, protocols, and
systems~\cite{aceto2018comprehensive, aceto_internet_2015}.  Understanding the
censorship mechanism can also help develop circumvention
techniques~\cite{winter2012great, chai2019importance, satija2021blindtls}.
\vskip 0.5em
Aside from these technical perspectives, there have been pursuits to gauge its
social, political, cultural, and religious
implications~\cite{shishkina2018internet, meserve2018google,
chen2000pornography}. These works reveal the complexity and the intricacy of 
the Internet censorship, which sometimes challenges conventional wisdom
given its prevalence among countries, polities, cultures, and religions 
of a great spectrum~\cite{aryan2013internet, nabi2013anatomy, singh2017characterizing,
yadav2018light, ng2018detecting,
meserve2018google, bock2021even, padmanabhan2021multi, ververis2021understanding}.
\end{revisiontext}

\noindent
	Internet censorship is a complex global phenomenon. It can be argued that in democratic
	countries Internet censorship may be less frequent than in non-democratic countries; however, it is
	certainly an overstatement to insist that there is no Internet censorship in democratic
	countries. Figure 8 in Niaki et al. clearly exhibits this~\cite{niaki2020iclab}.
	Meserve and Pemstein provide an investigation on Internet censorship in democratic
	countries with an aim to answer the question, ``how do democracies censor the internet,
	and why?~\cite{meserve2018google}'' Censored Planet~\cite{sundara_raman_censored_2020} queries the endpoints around the globe both for these reasons and for comparison.
 
    Arguably, there are more peer-reviewed studies
	about Internet censorship in non-democratic countries where Internet censorship is
	more prevalent. These studies include multiple studies on
	the Great Firewall of China, on Internet censorship in Iran, Myanmar, and Pakistan, 
	and on censorship mechanisms
	adopted in these countries~\cite{aryan2013internet, nabi2013anatomy, singh2017characterizing,
	ng2018detecting, bock2021even, padmanabhan2021multi}. 

	However, the censorship phenomenon is too complex
	for us to give a fair treatment in this article. Rather, this article is on automatic detection techniques
	of Internet censorship. The aim here is to investigate methods that could provide better tools to keen "observers." 


\commentno{r2xmlr}
\subsection{\refcomm{r2}{r2xmlr}. On Application of XLM-R}

\comment{%
A figure might clarify the approach based on XLM-R that is used to encode the
	text fields.%
}
\response{
	In Section 3.1, we added a figure to the paper in order to make the description of the tokenizer clearer. The added text and figure 
	are as follows:
}

\begin{revisiontext}
		Figure~\ref{fig:xlmr} illustrates the processing pipeline
		for these data fields. 

		\vskip 1em

		% \begin{figure}[!htbp]
			\centering
			\begin{adjustbox}{max width=\textwidth}
			\begin{tikzpicture}
				\tikzset{
					node distance=0.2in and 0.2in,
					inout/.style={rectangle, draw, dashed, black, align=center, font=\footnotesize,
					minimum height=0.25in, rounded corners=0pt},
					box/.style={rectangle, draw, solid, black, drop shadow, fill=white, align=center, font=\footnotesize,
					minimum height=0.25in, rounded corners=3pt}
				}
				\node[inout](url){\code{test\_url} field};
				\node[inout, below=of url](resp){\code{response} field};
				\node[box, right=of resp, yshift=0.25in](token){Extract text token\\using XML-R};
				\node[box, right=of token](dict){Form \\ token dictionary};
				\node[box, right=of dict](xmlr){Index text tokens  from\\pretrained XML-R};
				\node[box, right=of xmlr](filter){Filter out\\token indices\\per the dictionary};
				\node[inout, right=of filter](vector){Token index \\vectors};
		
				\draw[-latex](url) -- (token);
				\draw[-latex](resp) -- (token);
				\draw[-latex](token) -- (dict);
				\draw[-latex](dict) -- (xmlr);
				\draw[-latex](xmlr) -- (filter);
				\draw[-latex](filter) -- (vector);
		
				
			\end{tikzpicture}
			\end{adjustbox}
			\captionof{figure}{\sffamily Multilingual data processing of the \code{test\_url} and \code{response} fields and dimensionality reduction via 
			a pretrained XLM-R model~\cite{conneau2020unsupervised}. 
			The \code{response} field can contain natural language text and program code. To reduce the size of the encoding vectors, We
			filter out those with low frequency, such as, those do not appear in our data (i.e., frequency is 0) or rarely appear depending
			on the constraint of the available computational resources. In this work, by filtering out tokens with frequency of 0, we reach
			sufficiently small embedding vectors of length of 6,813.}
			\label{fig:xlmr}	
			
		% \end{figure}
	\end{revisiontext}


\commentno{r2ct}
\subsection{\refcomm{r2}{r2ct}. On Context Vector of the Model}

\comment{%
	Please describe in further detail the context vector.%
}
\response{
	This is great advice. In Section 3.2, we added the following sentences and revised the discussion about the attention score as follows:
}
\begin{revisiontext}
	$\ldots$

	$\ldots$
The weighted context vector here is to capture
the importance of different source-side information (e.g., which element in the state
vector) for predicting the probability of a particular token in the vocabulary~\cite{luong2015effective}.
We shall give a more detailed treatment of the context vector below (See the discussion about  Equation~\eqref{eq:attention}).
	$\ldots$

	$\ldots$

	The decoder is a sequence of bidirectional Gated Recurrent Unit Cells. We enhance
	it with an attention mechanism~\cite{niu2021review}, in particular, the ``dot'' 
	attention mechanism~\cite{luong2015effective}. 
	Instead of using fixed
	neuron weights, the attention mechanism allows us to enhance the 
	effect of some parts of the input data while diminishing other parts for predicting
	token probabilities via attention scores. 
	In one
	direction, each token in the input sequence is processed through the GRU cells.
	In the other direction, we calculate attention scores. Attention scores are
	computed using a dot product~\cite{raff_inside_2021}
	
	\begin{equation} \label{eq:attention}
	score(h_t, c_t) = \frac{h_t^T \cdot c_t}{\sqrt{H}}
	\end{equation}
	
	\noindent with values of $h_t$ taken from the state produced at step $t$ by the
	encoder, $h_t^T$ is $h_t$'s transpose, $c_t$ is the context, 
	and $H$ is the
	input size used for the GRU Cell. We compute $c_t$ as the decoder output at step $t$.
	We use the attention scores to weight the input sequence at each step of the decoding process.
	
\end{revisiontext}	

\commentno{r2bm}
\subsection{\refcomm{r2}{r2bm}. On Baseline Model}

\comment{%
	It would be interesting to use another simpler approach as the baseline
	method to assess how typical/naive classifier methods would perform in this
	problem. Although the comparison with image classification is useful, a
	naiver approach would serve better to the purpose of motivating the need for
	the complex combination of techniques that are proposed (i.e., the need for
	representation learning, sequence encoding, etc.).%
}
\response{
	This is an excellent suggestion. Typically, to use a simple model, we need
	to construct tabular data from the Internet measurement data where each column 
	is a data feature and each row is a feature vector for the corresponding 
	measurement record. 

	The tabular data are not readily available. We must decide what features to 
	construct and extract from the measurement data. By comparing existing features, 
	the best performing features in prior works are the image representation of 
	the measurement records~\cite{raman_measuring_2020, niaki2020iclab}. 
	In our baseline model, we adopt the image representations
	of the measurement records extracted using a pretrained neural network. Typically,
	neural networks are adopted as a classifier for the image data~\cite{hemalatha_efficient_2021,chen2020software}. 
	Our baseline model is built upon this. As such, we believe that a simple baseline
	model, such as, a Random Forest model using the features like page length and 
	term frequency vectors are unnecessary since these features are already shown to
	yield large false positives in prior researches on Internet censorship 
	detections~\cite{yadav2018light, raman2020measuring}. 
	
	In our response to Review~\ref{r1}'s comment~R\ref{r1}.\ref{r1bm}, 
	we have a detailed discussion about the baseline model. We hope our responses are
	adequate to address the reviewer's concern. 




}

